Maximum Likelihood Training for Score-Based Diffusion ODEs by High-Order Denoising Score Matching

Score-based generative models have excellent performance in terms of generation quality and likelihood. They model the data distribution by matching a parameterized score network with first-order data score functions. The score network can be used to define an ODE ("score-based diffusion ODE") for exact likelihood evaluation. However, the relationship between the likelihood of the ODE and the score matching objective is unclear. In this work, we prove that matching the first-order score is not sufficient to maximize the likelihood of the ODE, by showing a gap between the maximum likelihood and score matching objectives. To fill up this gap, we show that the negative likelihood of the ODE can be bounded by controlling the first, second, and third-order score matching errors; and we further present a novel high-order denoising score matching method to enable maximum likelihood training of score-based diffusion ODEs. Our algorithm guarantees that the higher-order matching error is bounded by the training error and the lower-order errors. We empirically observe that by high-order score matching, score-based diffusion ODEs achieve better likelihood on both synthetic data and CIFAR-10, while retaining the high generation quality.

==> fgkgtjmwskwbymryhxmxswbkzvkyvmcj/1-intro.tex <==
\section{Introduction}
\begin{figure}[t]
	\centering
	\begin{minipage}{0.32\linewidth}
		\centering
			\includegraphics[width=\linewidth]{figures/data_logpx.pdf}\\
\small{(a) Data \\ \ }
	\end{minipage}
	\begin{minipage}{0.32\linewidth}
		\centering		
 	\includegraphics[width=\linewidth]{figures/VE_logpx.pdf}\\
\small{(b) {\ode}\\ (first-order SM) %
}
   \end{minipage}
\begin{minipage}{0.32\linewidth}
		\centering		
 	\includegraphics[width=\linewidth]{figures/VE_third_logpx.pdf}\\
\small{(c) {\ode}\\ (third-order SM) %
}
   \end{minipage}
   \vspace{-.05in}
	\caption{\label{fig:mog_intro}
An 1-D mixture-of-Gaussians data distribution (a) and \ode 's density (b,c). (b): {\ode} trained by minimizing the first-order score matching (SM) objective in~\cite{song2021maximum}, which fails to estimate the density around $x=-0.25$. (c): {\ode} trained by minimizing our proposed third-order SM objective, which approximates the data density well.}
\vspace{-.15in}
\end{figure}

Score-based generative models (SGMs) have shown promising %
performance in both sample quality and likelihood evaluation~\cite{song2020score,vahdat2021score,dockhorn2021score,kingma2021variational}, with applications %
on many tasks, such as image generation~\cite{dhariwal2021diffusion,meng2021sdedit}, speech synthesis~\cite{chen2020wavegrad,kong2020diffwave}, shape generation~\cite{luo2021diffusion,zhou20213d} and lossless compression~\cite{kingma2021variational}. SGMs define a forward diffusion process by a stochastic differential equation (SDE) that gradually perturbs the data distribution to a simple noise distribution. The forward diffusion process has an equivalent reverse-time process with analytical form~\cite{anderson1982reverse}, which depends on the \textit{score function} (the gradient of the log probability density) of the forward process at each time step. SGMs learn a parameterized neural network (called ``score model'')~\cite{song2020sliced,song2019generative,song2020improved,song2020score} to estimate the score functions, and further define probabilistic models by the score model.

Two types of probabilistic models are proposed with the learned score model. One is the score-based diffusion SDE (\citet{song2020score}, ``\sde'' for short), which is defined by approximately reversing the diffusion process from the noise distribution by the score model and it can generate high-quality samples. The other is the score-based diffusion ordinary differential equation (\citet{song2020score, song2021maximum}, ``\ode'' for short), which is defined by approximating the probability flow ODE~\cite{song2020score} of the forward process whose marginal distribution is the same as the forward process at each time. 
\ode s can be viewed as continuous normalizing flows~\cite{chen2018neural}. Thus, unlikely SDEs, they can compute exact likelihood by ODE solvers~\cite{grathwohl2018ffjord}.

In practice, the score models are trained by minimizing an objective of a time-weighted combination of score matching losses~\cite{hyvarinen2005estimation,vincent2011connection}. It is proven that for a specific weighting function, minimizing the score matching objective is equivalent to maximizing the likelihood of the {\sde}~\cite{song2021maximum}.
However, minimizing the score matching objective does not necessarily maximize the likelihood of the \ode.
This is problematic since \ode s are used for likelihood estimation. 
In fact, \ode s trained with the score matching objective may even fail to estimate the likelihood of very simple data distributions, as shown in Fig.~\ref{fig:mog_intro}.

In this paper, we systematically analyze the relationship between the score matching objective and the maximum likelihood objective of {\ode}s, and present a new algorithm to learn \ode s via maximizing likelihood. Theoretically, we derive an equivalent form of the KL divergence\footnote{Maximum likelihood estimation is equivalent to minimizing a KL divergence.} between the data distribution and the \ode~distribution, which explicitly reveals the gap between the KL divergence and the original first-order score matching objective. 
Computationally, as directly optimizing the equivalent form requires an ODE solver, which is time-consuming~\cite{chen2018neural}, we derive an upper bound of the KL divergence by controlling the approximation errors of the first, second, and third-order score matching. The optimal solution for this score model by minimizing the upper bound is still the data score function, so the learned score model can still be used for the sample methods in SGMs (such as PC samplers in~\cite{song2020score}) to generate high-quality samples.

Based on the analyses, we propose a novel high-order denoising score matching algorithm to train the score models, which theoretically guarantees bounded approximation errors of high-order score matching. We further propose some scale-up techniques for practice. Our experimental results empirically show that the proposed training method can improve the likelihood of \ode s on both synthetic data and CIFAR-10, while retaining the high generation quality.












\section{Score-Based Generative Models}
\label{sec:background}
We first review the dynamics and probability distributions defined by SGMs. The relationship between these dynamics is illustrated in Fig.~\ref{fig:relationship}(a). 
\subsection{\sde s and Maximum Likelihood Training}
Let $q_0(\x_0)$ denote an unknown $d$-dimensional data distribution. SGMs 
define an SDE from time $0$ to $T$ (called ``forward process") with $\x_0\sim q_0(\x_0)$ and
\begin{equation}
\label{eqn:forward_sde}
    \dxv_t=\fv(\x_t,t)\dt+g(t)\dwv_t,
\end{equation}
where $\x_t$ is the solution at time $t$, $\fv(\cdot,t):\R^d\rightarrow\R^d$ and $g(t)\in\R$ are fixed functions such that the marginal distribution of $\x_T$ is approximately $\N(\x_T|\vect{0},\sigma_T^2\Iv)$ with $\sigma_T>0$, and $\wv_t\in\R^d$ is the standard Wiener process. Let $q_t(\x_t)$ denote the marginal distribution of $\x_t$. Under some regularity conditions, the forward process in Eqn.~\eqref{eqn:forward_sde} has an equivalent reverse process~\cite{anderson1982reverse} from time $T$ to $0$ with $\x_T\sim q_T(\x_T)$:
\begin{equation}
\label{eqn:reverse_sde_q}
    \dxv_t=[\fv(\x_t,t)-g(t)^2\nabla_{\x}\log q_t(\x_t)]\dt+g(t)\dm \bar{\wv}_t,
\end{equation}
where $\bar{\wv}_t$ is a standard Wiener process in the reverse-time. The marginal distribution of $\x_t$ in the reverse process in Eqn.~\eqref{eqn:reverse_sde_q} is also $q_t(\x_t)$. The only unknown term in Eqn.~\eqref{eqn:reverse_sde_q} is the time-dependent score function $\nabla_{\x}\log q_t(\x_t)$. SGMs use a neural network $\s_\theta(\x_t,t)$ parameterized by $\theta$ to estimate the score function for all $\x_t\in\R^d$ and $t\in[0,T]$. The neural network is trained by matching $\s_\theta(\x_t,t)$ and $\nabla_{\x}\log q_t(\x_t)$ with
the \emph{score matching objective}:
\begin{equation*}
\begin{aligned}
    &\Jc_{\SM}(\theta;\lambda(\cdot))\\
    &\coloneqq  \frac{1}{2}\int_0^T\lambda(t)\E_{q_t(\x_t)}\Big[\|\s_\theta(\x_t,t)-\nabla_{\x}\log q_t(\x_t)\|_2^2\Big]\dt,
\end{aligned}
\end{equation*}
where $\lambda(\cdot)>0$ is a weighting function. By approximating the score function with $\s_\theta(\x_t,t)$, SGMs define a parameterized reverse SDE from time $T$ to time $0$ with probability at each time $t$ denoted as $p^{\SDE}_t(\x_t)$ (omitting the subscript $\theta$). In particular, suppose $\x_T\sim p^{\SDE}_T(\x_T)=\Nc(\x_T|\vect{0},\sigma^2_T\Iv)$, the parameterized reverse SDE is defined by
\begin{equation}
\label{eqn:reverse_sde_p}
    \dxv_t=[\fv(\x_t,t)-g(t)^2\s_\theta(\x_t,t)]\dt+g(t)\dm \bar{\wv}_t,
\end{equation}
where the marginal distribution of $\x_t$ is $p^{\SDE}_t(\x_t)$. By solving the parameterized reverse SDE, SGMs achieve excellent sample quality in many tasks~\cite{song2020score,dhariwal2021diffusion}. Moreover, the KL divergence between $q_0(\x_0)$ and $p_0^{\SDE}(\x_0)$ can be bounded by the score matching error with the weight $g(\cdot)^2$~\cite{song2021maximum}:
\begin{equation}
\label{eqn:sde_elbo}
    \kl{q_0}{p_0^{\SDE}}\leq \kl{q_T}{p_T^{\SDE}}+\Jc_{\SM}(\theta;g(\cdot)^2).
\end{equation}
Therefore, minimizing $\Jc_{\SM}(\theta;g(\cdot)^2)$ is equivalent to maximum likelihood training of $p^{\SDE}_0$. In the rest of this work, we mainly consider the maximum likelihood perspective, namely $\lambda(\cdot)=g(\cdot)^2$, and denote $\Jc_{\SM}(\theta)\coloneqq\Jc_{\SM}(\theta;g(\cdot)^2)$.



\subsection{\ode s and Exact Likelihood Evaluation}
The parameterized \sde~cannot be used for exact likelihood evaluation, because we cannot evaluate $p_0^{\SDE}(\x_0)$ exactly for a given point $\x_0\in\R^d$. However, every SDE has an associated \textit{probability flow ODE}~\cite{song2020score} whose marginal distribution at each time $t$ is the same as that of the SDE. Unlike SDEs, the log-density of the ODE can be exactly computed by the ``Instantaneous Change of Variables"~\cite{chen2018neural}. Particularly, the probability flow ODE of the forward process in Eqn.~\eqref{eqn:forward_sde} is
\begin{equation}
\label{eqn:forward_ode}
    \frac{\dxv_t}{\dt}=\hv_q(\x_t,t)\coloneqq\fv(\x_t,t)-\frac{1}{2}g(t)^2\nabla_{\x}\log q_t(\x_t).
\end{equation}
If we start from $\x_0\sim q_0(\x_0)$, the distribution of each $\x_t$ during the ODE trajectory is also $q_t(\x_t)$.
Note that the only unknown term in Eqn.~\eqref{eqn:forward_ode} is also the score function $\nabla_{\x}\log q_t(\x_t)$. By approximating the score function with $\s_\theta(\x_t,t)$, SGMs define a parameterized ODE called ``score-based diffusion ODE'' (\ode) with probability $p^{\ODE}_t(\x_t)$ (omitting the subscript $\theta$) at each time $t$. In particular, suppose $\x_T\sim p_T^{\ODE}(\x_T)=p_T^{\SDE}(\x_T)=\N(\x_T|\vect{0},\sigma_T^2\Iv)$, the {\ode} is defined by
\begin{equation}
\label{eqn:score_ode}
    \frac{\dxv_t}{\dt}=\hv_p(\x_t,t)\coloneqq\fv(\x_t,t)-\frac{1}{2}g(t)^2\s_\theta(\x_t,t),
\end{equation}
where the marginal distribution of $\x_t$ is $p_t^{\ODE}(\x_t)$. By the ``Instantaneous Change of Variables"~\cite{chen2018neural}, $\log p_t^{\ODE}(\x_t)$ of $\x_t$ can be computed by integrating:
\begin{equation}
\label{eqn:change_of_variable_score_ode}
    \frac{\dm \log p^{\ODE}_t(\x_t)}{\dt}=-\tr(\nabla_{\x}\hv_p(\x_t,t)).
\end{equation}
If $\s_\theta(\x_t,t)\equiv\nabla_{\x}\log q_t(\x_t,t)$ for all $\x_t\in\R^d$ and $t\in[0,T]$, we have $\hv_p(\x_t,t)=\hv_q(\x_t,t)$. In this case, for all $\x_0\in\R^d$, $\log p_0^{\ODE}(\x_0)-\log q_0(\x_0)=\log p_T^{\ODE}(\x_T)-\log q_T(\x_T)\approx 0$ (because $q_T\approx p^{\ODE}_T$), where $\x_T$ is the point at time $T$ given by Eqn.~\eqref{eqn:forward_ode} starting with $\x_0$ at time $0$. Inspired by this, SGMs use the {\ode} with the score model for exact likelihood evaluations.




However, if $\s_\theta(\x_t,t)\neq\nabla_{\x}\log q_t(\x_t,t)$, there is no theoretical guarantee for bounding $\kl{q_0}{p_0^{\ODE}}$ of {\ode}s by the score matching objective $\Jc_{\SM}(\theta)$. As a result, after minimizing $\Jc_{\SM}(\theta)$, \citet{song2021maximum} find that the {\sde} of the ``Variance Exploding'' type~\cite{song2020score} achieves state-of-the-art sample quality, but the log-likelihood of the corresponding {\ode} is much worse (e.g., $\approx3.45$ bits/dim on CIFAR-10 dataset) than that of other comparable models (e.g., $\approx3.13$ bits/dim of the "Variance Preserving" type~\cite{song2020score}). Such observations pose a serious concern on the behavior of the likelihood of $p^{\ODE}_0$, which is not well understood. We aim to provide a systematical analysis in this work.



==> fgkgtjmwskwbymryhxmxswbkzvkyvmcj/2-ode_likelihood.tex <==
\section{Relationship between Score Matching and KL Divergence of \ode s}
\label{sec:ode_likelihood}

\begin{figure*}[t]
\centering
	\begin{minipage}{0.53\linewidth}
\begin{tikzpicture}[node distance=1.0cm]
    \draw [decorate, decoration = {brace,
            raise=5pt,
            amplitude=5pt,
            aspect=0.5},thick] (0, -2) --  (0,0)
    node(q)[pos=0.5,left=10pt,black]{$q_t(\x_t)$};
    \node(fs)[smalltext, right of=q, yshift=1.0cm, anchor=west, xshift=-0.2cm] {\scriptsize Forward SDE (Eqn.\eqref{eqn:forward_sde})};
    \node(rs)[smalltext, right of=q, anchor=west, xshift=-0.2cm] {\scriptsize Reverse SDE (Eqn.\eqref{eqn:reverse_sde_q})};
    \node(qode)[smalltext, right of=q, yshift=-1.0cm, anchor=west, xshift=-0.2cm] {\scriptsize Probability flow ODE (Eqn.\eqref{eqn:forward_ode})};
    \node(psde)[right of=rs, anchor=west, xshift=3.5cm]{$p_t^{\SDE}(\x_t)$};
    \node(pode)[right of=qode, xshift=3.cm, anchor=west]{$p_t^{\ODE}(\x_t)$};
    \draw [arrow] (rs) -> (psde);
    \node(Def)[smalltext, below of=psde, xshift=-2.35cm, yshift=0.5cm] {\scriptsize approximate $\nabla_{\x}\log q_t$ by $\s_\theta$};
    \draw [arrow] (qode) -> (pode);
    \node(Def)[smalltext, above of=psde, xshift=-2.3cm, yshift=-0.7cm] {\scriptsize Eqn.~\eqref{eqn:reverse_sde_p}};
    \node(Def)[smalltext, below of=pode, xshift=-1.85cm, yshift=0.7cm] {\scriptsize Eqn.~\eqref{eqn:score_ode}};
    \node(pneq)[rotate=90, below of=psde, xshift=-0.5cm, yshift=1.0cm]{$\neq$};
    \node(Def)[smalltext, below of=psde, xshift=0.9cm, yshift=0.5cm] {\scriptsize (Appendix.~\ref{appendix:distribution_gap})};
\end{tikzpicture}\\
	\centering
    \small{(a) Relationship between $q_t$, $p_t^{\SDE}$ and $p_t^{\ODE}$.}
	\end{minipage}
		\begin{minipage}{0.45\linewidth}
		\centering
        \begin{tikzpicture}[node distance=1.0cm]
        \node(klsde) {$\kl{q_0}{p_0^{\SDE}}$};
        \node(klode)[right of=klsde, xshift=2.1cm] {$\kl{q_0}{p_0^{\ODE}}$};
        \node(sdeup)[below of=klsde, yshift=-0.4cm]{$\Jc_{\SM}(\theta)$};
        \draw [dasharrow] (klsde.south) -> (sdeup.north);
        \node(odeup)[below of=klode, yshift=-0.4cm]{$\sqrt{\Jc_{\SM}(\theta)}\cdot\sqrt{\Jc_{\FISH}(\theta)}$};
        \draw [arrow] (klode.south) -> (odeup.north);
        \node(sdesm)[below of=sdeup, yshift=-0.2cm]{\scriptsize first-order SM};
        \node(odesm1)[below of=odeup, xshift=-0.9cm, yshift=-0.2cm]{\scriptsize first-order SM};
        \node(odesm2)[below of=odeup, xshift=-0.1cm, anchor=west, yshift=-0.2cm]{\scriptsize second, third-order SM};
        \node(thrm)[below of=odesm2, yshift=0.6cm]{\scriptsize (Theorem~\ref{thrm:second}, \ref{coro:second_trace}, \ref{thrm:third})};
        \draw [dasharrow] (sdeup.south) -> (sdesm.north);
        \draw [dasharrow] (odesm1.north |- odeup.south) -> (odesm1.north);
        \draw [arrow] (odesm2.north |- odeup.south) -> (odesm2.north);
        \node(Def)[below of=klsde, xshift=-0.1cm, yshift=0.35cm, anchor=east]{\scriptsize \cite{song2021maximum}};
        \node(Def)[below of=klode, xshift=0.1cm, anchor=west, yshift=0.35cm]{\scriptsize (Theorem~\ref{thrm:kl-ode} \& Eqn.~\eqref{eqn:cauchy_ode})};
        \node(Def)[below of=klode, xshift=-1.55cm, yshift=0.35cm] {\scriptsize $\leftarrow$minimizing upper bound$\rightarrow$};
        \node(Def)[above of=odesm2, yshift=-0.4cm, xshift=0.8cm]{\scriptsize (Theorem~\ref{thrm:fisher_bound})};
        \end{tikzpicture}\\
        \small{(b) Relationship between SM objectives and KL divergence.}
		\end{minipage}
\centering
\caption{An illustration of the theoretical analysis of score-based generative models and score matching (SM) objectives.\label{fig:relationship}}
\vspace{-.1in}
\end{figure*}


The likelihood evaluation needs the distribution $p_0^{\ODE}$ of {\ode}s, which is usually different from the distribution $p^{\SDE}_0$ of {\sde}s (see Appendix~\ref{appendix:distribution_gap} for detailed discussions). Although the score matching objective $\Jc_{\SM}(\theta)$ can upper bound the KL divergence of {\sde}s (up to constants) according to Eqn.~\eqref{eqn:sde_elbo}, it is not 
enough to upper bound the KL divergence of {\ode}s. To the best of our knowledge, there is no theoretical analysis of the relationship between the score matching objectives and the KL divergence of {\ode}s.



In this section, we reveal the relationship between the first-order score matching objective $\Jc_{\SM}(\theta)$ and the KL divergence $\kl{q_0}{p_0^{\ODE}}$ of {\ode}s, and upper bound $\kl{q_0}{p_0^{\ODE}}$ by involving high-order score matching. Fig.~\ref{fig:relationship} demonstrates our theoretical analysis and the connection with previous works.



\subsection{KL Divergence of \ode s}



In the following theorem, we propose a formulation of the KL divergence $\kl{q_0}{p_0^{\ODE}}$ by integration, which shows that there is a non-zero gap between the KL divergence and the score matching objective $\Jc_{\SM}(\theta)$.%


\begin{theorem}[Proof in Appendix~\ref{appendix:thrm_kl_ode}]
\label{thrm:kl-ode}
Let $q_0$ be the data distribution and $q_t$ be the marginal distribution at time $t$ through the forward diffusion process defined in Eqn.~\eqref{eqn:forward_sde}, and $p^{\ODE}_t$ be the marginal distribution at time $t$ through the {\ode} defined in Eqn.~\eqref{eqn:score_ode}. Under some regularity conditions in Appendix~\ref{appendix:assumptions}, we have
\begin{equation*}
\begin{medsize}
\begin{aligned}
    \nonumber
    \kl{q_0}{p^{\ODE}_0}\!&=\!\kl{q_T}{p^{\ODE}_T}+\Jc_{\ODE}(\theta)\\
    &=\!\!\!\!\!\!\underbrace{\kl{q_T}{p^{\ODE}_T}+\Jc_{\SM}(\theta)}_{\text{upper bound of $\kl{q_0}{p_0^{\SDE}}$ in Eqn.~\eqref{eqn:sde_elbo}}}\!\!\!+\ \Jc_{\DIFF}(\theta),
\end{aligned}
\end{medsize}
\end{equation*}
where
\begin{small}
\begin{align}
    \nonumber
    \Jc_{\ODE}(\theta)\!&\coloneqq\!\frac{1}{2}\!\int_0^T \!\!\!g(t)^2\E_{q_t(\x_t)}\!\Big[(\s_\theta(\x_t,t)\!-\!\nabla_{\x}\log q_t(\x_t))^\top\\ 
    &(\nabla_{\x}\log p_t^{\ODE}(\x_t)\!-\!\nabla_{\x}\log q_t(\x_t))\Big]\dt,
    \label{eqn:kl_ode}\\
    \nonumber
    \Jc_{\DIFF}(\theta)\!&\coloneqq\!\frac{1}{2}\int_0^T \!\!\!g(t)^2\E_{q_t(\x_t)}\!\Big[(\s_\theta(\x_t,t)\!-\!\nabla_{\x}\log q_t(\x_t))^\top\\
    &(\nabla_{\x}\log p_t^{\ODE}(\x_t)\!-\!\s_\theta(\x_t,t))\Big]\dt.
    \label{eqn:J_diff}
\end{align}
\end{small}%
\end{theorem}
As $p^{\ODE}_T$ is fixed, minimizing $\kl{q_0}{p^{\ODE}_0}$ is equivalent to minimizing $\Jc_{\ODE}(\theta)$, which includes $\Jc_{\SM}(\theta)$ and $\Jc_{\DIFF}(\theta)$. While minimizing $\Jc_{\SM}(\theta)$ reduces the difference between $\s_\theta(\cdot,t)$ and the data score $\nabla_{\x}\log q_t$, it cannot control the error of $\Jc_{\DIFF}(\theta)$, which includes the difference between $\s_\theta(\cdot,t)$ and the model score $\nabla_{\x}\log p_t^{\ODE}$. As we show in Fig.~\ref{fig:mog_intro}, only minimizing $\Jc_{\SM}(\theta)$ may cause problematic model density of the {\ode}.




\subsection{Bounding the KL Divergence of \ode s by High-Order Score Matching Errors}
\label{sec:kl_bounding}
The KL divergence in Theorem~\ref{thrm:kl-ode} includes the model score function $\nabla_{\x}\log p^{\ODE}_t(\x_t)$, which needs ODE solvers to compute (see Appendix.~\ref{appendix:change_of_score} for details) and thus is hard to scale up. Below we derive an upper bound of $\kl{q_0}{p_0^{\ODE}}$ by involving high-order score matching, which can avoid the computation of $\nabla_{\x}\log p^{\ODE}_t(\x_t)$. Specifically, we show that by bounding the first, second and third-order score matching errors for $\s_\theta, \nabla_{\x}\s_\theta$ and $\nabla_{\x}\tr(\nabla_{\x}\s_\theta)$ with the corresponding order score functions\footnote{In this work, we refer to $\nabla_{\x}^2\log q_t(\x_t)$ as the second-order score function of $q_t$, and $\nabla_{\x}\tr(\nabla_{\x}^2\log q_t(\x_t))$ as the third-order score function of $q_t$.} of $q_t$, we can further upper bound $\kl{q_0}{p_0^{\ODE}}$.


Let $\fisher{q}{p}\coloneqq \E_{q(\x)}\|\nabla_{\x}\log p(\x)-\nabla_{\x}\log q(\x)\|_2^2$ denote the Fisher divergence between two distributions $q$ and $p$. Define
\begin{equation}
    \Jc_{\FISH}(\theta)\coloneqq \frac{1}{2}\int_0^T g(t)^2\fisher{q_t}{p^{\ODE}_t}\dt.
\end{equation}
By straightforwardly using Cauchy-Schwarz inequality for Eqn.~\eqref{eqn:kl_ode}, we have
\begin{equation}
\label{eqn:cauchy_ode}
    \Jc_{\ODE}(\theta)\leq \sqrt{\Jc_{\SM}(\theta)}\cdot\sqrt{\Jc_{\FISH}(\theta)}.
\end{equation}%
The upper bound shows that we can minimize the KL divergence $\kl{q_0}{p_0^{\ODE}}$ of {\ode} by minimizing $\Jc_{\SM}(\theta)$ and $\Jc_{\FISH}(\theta)$ simultaneously. %
When $\s_\theta(\x_t,t)\equiv\nabla_{\x}\log q_t(\x_t)$ for all $\x_t\in\R^d$ and $t\in[0,T]$, the equality holds and $\Jc_{\ODE}(\theta)=\Jc_{\SM}(\theta)=0$.

We can regard $\Jc_{\FISH}(\theta)$ as a weighted Fisher divergence between $q_t$ and $p_t^{\ODE}$ during $t\in[0,T]$. Directly computing the Fisher divergence also needs ODE solvers (see Appendix.\ref{appendix:change_of_score} for details) and is hard to scale up. To address this problem, we present the following theorem for bounding $\fisher{q_t}{p^{\ODE}_t}$, which introduces high-order score matching and avoids the computation costs of ODE solvers.

\begin{theorem}[Proof in Appendix~\ref{appendix:thrm_fisher_bound}]
\label{thrm:fisher_bound}
Assume that there exists $C>0$, such that for all $t\in [0,T]$ and $\x_t\in\R^d$, $\|\nabla_{\x}^2\log p_t^{\ODE}(\x_t)\|_2\leq C$ (where $\nabla^2$ denotes the second-order derivative (Hessian), and $\|\cdot\|_2$ is the spectral norm of a matrix). And assume that there exist $\delta_1,\delta_2,\delta_3>0$, such that for all $\x_t\in\R^d$, $t\in[0,T]$, $s_\theta(\x_t,t)$ satisfies

\begin{small}
\begin{equation*}
\begin{aligned}
    &\|\s_\theta(\x_t,t)-\nabla_{\x}\log q_t(\x_t)\|_2\leq\delta_1,\\
    &\|\nabla_{\x}\s_\theta(\x_t,t)-\nabla^2_{\x}\log q_t(\x_t)\|_F\leq\delta_2,\\
    &\|\nabla_{\x}\tr(\nabla_{\x}\s_\theta(\x_t,t))-\nabla_{\x}\tr(\nabla_{\x}^2\log q_t(\x_t))\|_2\leq\delta_3,
\end{aligned}
\end{equation*}
\end{small}%
where $\|\cdot\|_F$ is the Frobenius norm of matrices. Then there exists $U(t;\delta_1,\delta_2,\delta_3,C,q)\geq 0$ which depends on the forward process $q$ while is independent of $\theta$, such that $\fisher{q_t}{p^{\ODE}_t}\leq U(t;\delta_1,\delta_2,\delta_3,C,q)$. Moreover, for all $t\in[0,T]$, if $g(t)\neq 0$, then $U(t;\delta_1,\delta_2,\delta_3,C,q)$ is a strictly increasing function of $\delta_1$, $\delta_2$ and $\delta_3$, respectively.%

\end{theorem}
Theorem~\ref{thrm:fisher_bound} shows that by bounding the errors between $\s_\theta$, $\nabla_{\x}\s_\theta$ and $\nabla_{\x}\tr(\nabla_{\x}\s_\theta)$ with the first, second and third-order score functions of $q_t$, we can upper bound $\fisher{q_t}{p_t^{\ODE}}$ and then upper bound $\Jc_{\FISH}(\theta)$. As $\Jc_{\SM}(\theta)$ can also be upper bounded by the first-order score matching error of $\s_\theta$, we can further upper bound $\kl{q_0}{p_0^{\ODE}}$ by the first, second and third-order score matching errors.

Note that the high-order score matching for $\s_\theta$ is compatible for the traditional SGMs, because the optimal solution for $\s_\theta(\x_t,t)$ in the non-parametric limit is still $\nabla_{\x}\log q_t(\x_t)$. So after minimizing $\kl{q_0}{p_0^{\ODE}}$ by high-order score matching, we can still use $\s_\theta$ for the sample methods in SGMs, while directly minimizing $\kl{q_0}{p_0^{\ODE}}$ by exact likelihood ODE solvers cannot ensure that (see Appendix.~\ref{appendix:mle_scoreode_by_odesolver} for detailed reasons).

==> fgkgtjmwskwbymryhxmxswbkzvkyvmcj/3-high_order_SM.tex <==
\section{Error-Bounded High-Order Denoising Score Matching (DSM)}
\label{sec:high_order_SM}


The analysis in Sec.~\ref{sec:kl_bounding} shows that we can upper bound the KL divergence $\kl{q_0}{p_0^{\ODE}}$ of the {\ode} by controlling the first, second and third-order score matching errors of the score model $\s_\theta$ (and its corresponding derivatives) at each time $t\in[0,T]$. Inspired by this, we generalize the traditional denoising score matching (DSM)~\cite{vincent2011connection} to second and third orders to minimize the high-order score matching errors. In this section, we propose a novel high-order DSM method, such that the higher-order score matching error can be exactly bounded by the training error and the lower-order score matching error. All the proofs in this section are in Appendix.~\ref{appendix:proof_high_order_DSM}.


Without loss of generality, in this section, we focus on a fixed time $t\in(0,T]$, and propose the error-bounded high-order DSM method for matching the forward process distribution $q_t$ at the fixed time $t$. The whole training objective for the entire process by $t\in[0,T]$ is detailed in Sec.~\ref{sec:training}. Moreover, for SGMs, there commonly exist $\alpha_t\in\R$ and $\sigma_t\in\R_{>0}$, such that the forward process satisfies $q(\x_t|\x_0)=\N(\x_t|\alpha_t\x_0,\sigma_t^2\Iv)$ for $\x_0,\x_t\sim q_{t0}(\x_t,\x_0)$~\cite{song2020score}. Therefore, we always assume $q(\x_t|\x_0)=\N(\x_t|\alpha_t\x_0,\sigma_t^2\Iv)$  in the rest of this work.




\subsection{First-Order Denoising Score Matching}
We present some preliminaries on first-order denoising score matching~\cite{vincent2011connection,song2020score} in this section.

The first-order score matching objective $\Jc_{\SM}(\theta)$ needs the data score functions $\nabla_{\x}\log q_t(\x_t)$ for all $t\in[0,T]$, which are unknown in practice. To address this issue, SGMs leverage the denoising score matching method~\cite{vincent2011connection} to train the score models. For a fixed time $t$, one can learn a first-order score model $\s_1(\cdot,t;\theta):\R^d\rightarrow\R^d$ parameterized by $\theta$ which minimizes
\begin{equation*}
    \E_{q_t(\x_t)}\Big[\big\|\s_1(\x_t,t;\theta)-\nabla_{\x}\log q_t(\x_t)\big\|_2^2\Big],
\end{equation*}
by optimizing the (first-order) DSM objective:
\begin{equation}
\label{eqn:dsm-1-obj}
    \theta^*=\argmin_{\theta}\E_{\x_0,\epsilonv}\left[\frac{1}{\sigma_t^2}\big\|\sigma_t\s_1(\x_t,t;\theta)+\epsilonv\big\|_2^2\right],
\end{equation}
where $\epsilonv\sim\N(\vect{0},\Iv)$ and $\x_t=\alpha_t\x_0+\sigma_t\epsilonv$.


\subsection{High-Order Denoising Score Matching}
In this section, we generalize the first-order DSM to second and third orders for matching the second-order and third-order score functions defined in \cref{thrm:fisher_bound}.
We firstly present the second-order method below.
\begin{theorem}
\label{thrm:second}
(Error-Bounded Second-Order DSM) Suppose that $\hat\s_1(\x_t,t)$ is an estimation for the first-order data score function $\nabla_{\x}\log q_t(\x_t)$, then we can learn a second-order score model $\s_2(\cdot,t;\theta): \R^{d}\rightarrow\R^{d\times d}$ parameterized by $\theta$ which minimizes
\begin{equation*}
    \E_{q_t(\x_t)}\left[\left\|\s_2(\x_t,t;\theta)-\nabla^2_{\x}\log q_t(\x_t)\right\|_F^2\right],
\end{equation*}
by optimizing
{
\small
\begin{equation}
\label{eqn:dsm-2-obj}
\!\!\!\theta^*=\argmin_{\theta}\E_{\x_0,\epsilonv}\left[\frac{1}{\sigma_t^4}\big\|\sigma_t^2\s_2(\x_t,t;\theta)+\Iv-\ellv_1\ellv_1^\top\big\|^2_F\right],
\end{equation}
}%
where
\begin{equation}
\label{eqn:ell_1}
\begin{aligned}
    &\ellv_1(\epsilonv,\x_0,t)\coloneqq\sigma_t\hat\s_1(\x_t,t)+\epsilonv,\\
    &\x_t=\alpha_t\x_0+\sigma_t\epsilonv,\quad\epsilonv\sim \Nc(\vect{0},\Iv).
\end{aligned}
\end{equation}
Moreover, denote the first-order score matching error as $\delta_1(\x_t,t)\coloneqq\|\hat\s_1(\x_t,t)-\nabla_{\x}\log q_t(\x_t)\|_2$, then $\forall \x_t,  \theta$, the score matching error for $\s_2(\x_t,t;\theta)$ can be bounded by
\begin{equation*}
\begin{split}
    &\left\|\s_2(\x_t,t;\theta)-\nabla_{\x}^2\log q_t(\x_t)\right\|_F\\
    \leq\ &\left\|\s_2(\x_t,t,\theta)-\s_2(\x_t,t;\theta^*)\right\|_F+\delta_1^2(\x_t,t).
\end{split}
\end{equation*}
\end{theorem}
Theorem~\ref{thrm:second} shows that the DSM objective in problem~(\ref{eqn:dsm-2-obj}) is a valid surrogate for second-order score matching,
because the difference between the model score $\s_2(\x_t,t;\theta)$ and the true second-order score $\nabla^2_{\x}\log q_t(\x_t)$ can be bounded by the training error $\|\s_2(\x_t,t;\theta)-\s_2(\x_t,t;\theta^*)\|_F$ and the first-order score matching error $\delta_1(\x_t,t)$. Note that previous second-order DSM method proposed in~\citet{meng2021estimating} does not have such error-bounded property, and we refer to Sec.~\ref{sec:related} and Appendix~\ref{appendix:differ_high_order} for the detailed comparison. In addition, recent work~\citep[Theorem 3.3]{bao2022estimating} about the optimal covariance of the diffusion models considers the estimation error of the mean of the diffusion models, which is equivalent to our proposed error-bounded second-order DSM with considering the first-order score matching error.

The DSM objective in problem~(\ref{eqn:dsm-2-obj}) requires learning a matrix-valued function $\nabla^2_{\x}\log q_t(\x_t)$, but sometimes we only need the trace $\tr(\nabla^2_{\x}\log q_t(\x_t))$ of the second-order score function. 
Below we present a corollary for only matching the trace of the second-order score function.
\begin{corollary}
\label{coro:second_trace}
(Error-Bounded Trace of Second-Order DSM) We can learn a second-order trace score model $\s_2^{\text{trace}}(\cdot,t;\theta):\R^{d}\rightarrow\R$ which minimizes
\begin{equation*}
    \E_{q_t(\x_t)}\left[\left|\s_2^{\text{trace}}(\x_t,t;\theta)-\tr(\nabla_{\x}^2\log q_t(\x_t))\right|^2\right],
\end{equation*}
by optimizing
{\small
\begin{equation}
\label{eqn:dsm-2-trace-obj}
    \theta^*\!=\argmin_{\theta}\E_{\x_0,\epsilonv}\!\left[\frac{1}{\sigma_t^4}\Big|\sigma_t^2\s_2^{\text{trace}}(\x_t,t;\theta)\!+\!d\!-\!\|\ellv_1\|_2^2\Big|^2\right].
\end{equation}
}%
The estimation error for $\s_2^{\text{trace}}(\x_t,t;\theta)$ can be bounded by:
\begin{equation*}
 \begin{split}
&\left|\s_2^{\text{trace}}(\x_t,t;\theta)-\tr(\nabla^2_{\x}\log q_t(\x_t))\right|\\
\leq\ &\left|\s_2^{\text{trace}}(\x_t,t;\theta)-\s_2^{\text{trace}}(\x_t,t;\theta^*)\right|+\delta_1^2(\x_t,t).
 \end{split} 
\end{equation*}
\end{corollary}
Finally, we present the third-order DSM method. The score matching error can also be bounded by the training error and the first, second-order score matching errors.
\begin{theorem}
\label{thrm:third}
(Error-Bounded Third-Order DSM) Suppose that $\hat\s_1(\x_t,t)$ is an estimation for $\nabla_{\x}\log q_t(\x_t)$ and $\hat\s_2(\x_t,t)$ is an estimation for $\nabla^2_{\x}\log q_t(\x_t)$, then we can learn a third-order score model $\s_3(\cdot,t;\theta): \R^{d}\rightarrow\R^{d}$ which minimizes
\begin{equation*}
    \E_{q_t(\x_t)}\left[\left\|\s_3(\x_t,t;\theta)-\nabla_{\x}\tr(\nabla_{\x}^2\log q_t(\x_t))\right\|_2^2\right],
\end{equation*}
by optimizing
\begin{equation}
\label{eqn:dsm-3-obj}
\begin{split}
    &\theta^*=\argmin_{\theta}\E_{\x_0,\epsilonv}\left[\frac{1}{\sigma_t^6}\big\|\sigma_t^3\s_3(\x_t,t;\theta)+\ellv_3\big\|_2^2\right]
\end{split}
\end{equation}
where
\begin{equation}
\label{eqn:ell_3}
\begin{split}
    &\ellv_1(\epsilonv,\x_0,t)\coloneqq\sigma_t\hat\s_1(\x_t,t)+\epsilonv,\\
    &\ellv_2(\epsilonv,\x_0,t)\coloneqq\sigma_t^2\hat\s_2(\x_t,t)+\Iv,\\
    &\ellv_3(\epsilonv,\x_0,t)\coloneqq\left(\|\ellv_1\|_2^2\Iv-\tr(\ellv_2)\Iv-2\ellv_2\right)\ellv_1,\\
    &\x_t=\alpha_t\x_0+\sigma_t\epsilonv,\quad \epsilonv\sim\N(\vect{0},\Iv).
\end{split}
\end{equation}
Denote the first-order score matching error as $\delta_1(\x_t,t)\coloneqq\|\hat\s_1(\x_t,t)-\nabla_{\x}\log q_t(\x_t)\|_2$ and the second-order score matching errors as $\delta_2(\x_t,t)\coloneqq\|\hat\s_2(\x_t,t)-\nabla_{\x}^2\log q_t(\x_t)\|_F$ and $\delta_{2,\text{tr}}(\x_t,t)\coloneqq|\tr(\hat\s_2(\x_t,t))-\tr(\nabla_{\x}^2\log q_t(\x_t))|$. Then $\forall \x_t, \theta$, the score matching error for $\s_3(\x_t,t;\theta)$ can be bounded by:
\begin{equation*}
\begin{split}
    &\left\|\s_3(\x_t,t;\theta)-\nabla_{\x}\tr(\nabla_{\x}^2\log q_t(\x_t))\right\|_2\\
    \leq\ &\left\|\s_3(\x_t,t;\theta)-\s_3(\x_t,t;\theta^*)\right\|_2+\big(\delta_1^2+\delta_{2,\text{tr}}+2\delta_2\big)\delta_1^2
\end{split}
\end{equation*}
\end{theorem}
\cref{thrm:third} shows that the third-order score matching needs first-order score matching, second-order score matching and trace of second-order score matching. The third-order score matching error can also be bounded by the training error and the lower-order score matching errors. We believe that our construction for the error-bounded high-order DSM can be extended to even higher orders by carefully designing the training objectives. In this paper, we only focus on the second and third-order methods, and leave this extension for future work.

==> fgkgtjmwskwbymryhxmxswbkzvkyvmcj/4-related.tex <==
\vspace{-.1cm}
\section{Related Work}
\label{sec:related}
\vspace{-.05cm}
{\ode}s are special formulations of Neural ODEs (NODEs)~\cite{chen2018neural}, and our proposed method can be viewed as maximum likelihood training of NODEs by high-order score matching. Traditional maximum likelihood training for NODEs aims to match the NODE distribution at $t=0$ with the data distribution, and it cannot control the distribution between $0$ and $T$. \citet{finlay2020train} show that training NODEs by simply maximizing likelihood could result in unnecessary complex dynamics, which is hard to solve. Instead, our high-order score matching objective is to match the distributions between the forward process distribution and the NODE distribution at each time $t$, and empirically the dynamics is kind of smooth. Moreover, our proposed algorithm uses the Monto-Carlo method to unbiasedly estimate the objectives, which does not need any black-box ODE solvers. Therefore, our algorithm is suitable for maximum likelihood training for large-scale NODEs.

Recently, \citet{meng2021estimating} propose a high-order DSM method for estimating the second-order data score functions. However, the training objective of our proposed error-bounded high-order DSM is different from that of~\citet{meng2021estimating}. Our proposed algorithm can guarantee a bounded error of the high-order score matching exactly by  the lower-order estimation errors and the training error, while the score matching error raised by minimizing the objective in~\citet{meng2021estimating} may be unbounded, even when the lower-order score matching error is small and the training error of the high-order DSM is zero (see Appendix~\ref{appendix:differ_high_order} for detailed analysis). Moreover, our method can also be used to train a separate high-order score model in other applications, such as uncertainty quantification and Ozaki sampling presented in~\citet{meng2021estimating}.

==> fgkgtjmwskwbymryhxmxswbkzvkyvmcj/5-implementation.tex <==
\section{Training Score Models by High-Order DSM}
\label{sec:training}
Building upon the high-order DSM for a specific time $t$ (see  Sec.~\ref{sec:high_order_SM}), we present our algorithm to train {\ode}s in the perspective of maximum likelihood by considering all timesteps $t\in[0,T]$. 
Practically, we further leverage the ``noise-prediction'' trick~\cite{kingma2021variational,ho2020denoising} for variance reduction and the Skilling-Hutchinson trace estimator~\cite{skilling1989eigenvalues, hutchinson1989stochastic} to compute the involved high-order derivatives efficiently. The whole training algorithm is presented detailedly in Appendix.~\ref{appendix:training_algorithm}.

\subsection{Variance Reduction by Time-Reweighting}
\label{sec:variance_reduction}
Theoretically, to train score models for all $t\in[0,T]$, we need to integrate the DSM objectives in Eqn.~\eqref{eqn:dsm-1-obj}\eqref{eqn:dsm-2-obj}\eqref{eqn:dsm-2-trace-obj}\eqref{eqn:dsm-3-obj} from $t=0$ to $t=T$, which needs ODE solvers and is time-consuming. Instead, in practice, we follow the method in \cite{song2020score,ho2020denoising} which uses Monte-Carlo method to unbiasedly estimate the objectives by sample $t\in[0,T]$ from a proposal distribution $p(t)$, avoiding ODE solvers. The main problem for the Monte-Carlo method is that sometimes the sample variance of the objectives may be large due to the different value of $\frac{1}{\sigma_t}$. To reduce the variance, we take the time-reweighted objectives by multiplying $\sigma_t^2$,$\sigma_t^4$,$\sigma_t^6$ with the corresponding first, second, third-order score matching objectives at each time $t$, which is known as the ``noise-prediction'' trick~\cite{kingma2021variational,ho2020denoising} for the first-order DSM objective. Specifically, assume that $\x_0\sim q_0(\x_0)$, the time proposal distribution $p(t)=\Uc[0,T]$ is the uniform distribution in $[0,T]$,  the random noise $\epsilonv\sim\N(\vect{0},\Iv)$ follows the standard Gaussian distribution, and let $\x_t=\alpha_t\x_0+\sigma_t\epsilonv$. The training objective for the first-order DSM in Eqn.~\eqref{eqn:dsm-1-obj} through all $t\in[0,T]$ is
\begin{equation}
\label{eqn:dsm-1-final}
    \Jc_{\DSM}^{(1)}(\theta)\coloneqq \E_{t,\x_0,\epsilonv}\Big[\big\|\sigma_t\s_\theta(\x_t,t)+\epsilonv\big\|_2^2\Big],
\end{equation}
which empirically has low sample variance~\cite{song2020score,ho2020denoising}.

As for the second and third-order DSM objectives, we take $\hat\s_1(\x_t,t)\coloneqq \s_\theta(\x_t,t)$ for the first-order score function estimation, and $\hat\s_2(\x_t,t)\coloneqq \nabla_{\x}\s_\theta(\x_t,t)$ for the second-order score function estimation, and both disable the gradient computations for $\theta$ (which can be easily implemented by \texttt{stop\_gradient} or \texttt{detach}). The reason for disabling gradients is because the high-order DSM only needs the estimation values of the lower-order score functions, as shown in Theorem.~\ref{thrm:second} and \ref{thrm:third}. The training objectives through all $t\in[0,T]$ for the second-order DSM in Eqn.~\eqref{eqn:dsm-2-obj}, for the trace of second-order DSM in Eqn.~\eqref{eqn:dsm-2-trace-obj} and for the third-order DSM in Eqn.~\eqref{eqn:dsm-3-obj} are
\begin{equation*}
\begin{aligned}
    \Jc_{\DSM}^{(2)}(\theta)\!&\coloneqq\! \E_{t,\x_0,\epsilonv}\Big[\big\|\sigma_t^2\nabla_{\x}\s_\theta(\x_t,t)+\Iv-\ellv_1\ellv_1^\top\big\|_F^2\Big],\\
    \Jc_{\DSM}^{(2,\text{tr})}(\theta)\!&\coloneqq\! \E_{t,\x_0,\epsilonv}\Big[\big|\sigma_t^2\tr(\nabla_{\x}\s_\theta(\x_t,t))\!+\!d\!-\!\|\ellv_1\|_2^2\big|^2\Big],\\
    \Jc_{\DSM}^{(3)}(\theta)\!&\coloneqq\! \E_{t,\x_0,\epsilonv}\Big[\big\|\sigma_t^3\nabla_{\x}\!\tr(\nabla_{\x}\s_\theta(\x_t,t))\!+\ellv_3\big\|_2^2\Big],
\end{aligned}
\end{equation*}
respectively, where $\ellv_1,\ellv_3$ are the same as that in Eqn.~\eqref{eqn:ell_3}. Combining with the first-order objective in Eqn.~\eqref{eqn:dsm-1-final}, our final training objective is
\begin{equation}
\label{eqn:final_objective}
    \min_{\theta}\Jc_{\DSM}^{(1)}(\theta)+\lambda_1\left(\Jc_{\DSM}^{(2)}(\theta)+\Jc_{\DSM}^{(2,tr)}(\theta)\right)+\lambda_2\Jc_{\DSM}^{(3)}(\theta),
\end{equation}
where $\lambda_1,\lambda_2\geq0$ are hyperparameters, and we discuss in Appendix.~\ref{appendix:choose_lambda} for details.
\begin{remark}
Although as shown in Eqn.~\eqref{eqn:change_of_variable_score_ode}, we can exactly compute $\log p_0^{\ODE}(\x_0)$ for a given data point $\x_0$ via solving the ODE~\cite{chen2018neural, grathwohl2018ffjord}, this method is hard to scale up for the large neural networks used in SGMs. For example, it takes $2\sim 3$ minutes for evaluating $\log p^{\ODE}_0$ for a single batch of the {\ode} used in~\cite{song2020score}. Instead, our proposed method leverages Monte-Carlo methods to avoid the ODE solvers. %
\end{remark}


\subsection{Scalability and Numerical Stability}
As the second and third-order DSM objectives need to compute the high-order derivatives of a neural network and are expensive for high-dimensional data, we use the Skilling-Hutchinson trace estimator~\cite{skilling1989eigenvalues, hutchinson1989stochastic} to unbiasedly estimate the trace of the Jacobian~\cite{grathwohl2018ffjord} and the Frobenius norm of the Jacobian~\cite{finlay2020train}. The detailed objectives for high-dimensional data can be found in Appendix.~\ref{appendix:ubiased_estimation}.

In practice, we often face numerical instability problems for $t$ near to $0$. We follow~\citet{song2021maximum} to choose a small starting time $\epsilon>0$, and both of the training and the evaluation are performed for $t\in[\epsilon,T]$ instead of $[0,T]$. Note that the likelihood evaluation is still exact, because we use $p_{\epsilon}^{\ODE}(\x_0)$ to compute the log-likelihood of $\x_0$, which is still a well-defined density model~\cite{song2021maximum}.

==> fgkgtjmwskwbymryhxmxswbkzvkyvmcj/6-experiments.tex <==
\section{Experiments}
\vspace{-.05cm}

In this section, we demonstrate that our proposed high-order DSM algorithm can improve the likelihood of {\ode}s, while retaining the high sample quality of the corresponding {\sde}s. Particularly, we use the Variance Exploding (VE)~\cite{song2020score} type diffusion models, which empirically have shown high sample quality by the {\sde} but poor likelihood by the {\ode}~\cite{song2021maximum} when trained by minimizing the first-order score matching objective $\Jc_{\SM}(\theta)$. We implement our experiments by JAX~\cite{jax2018github},  which is efficient for computing the derivatives of the score models. In all experiments, we choose the start time $\epsilon=10^{-5}$, which follows the default settings in~\citet{song2020score}. In this section, we refer to ``first-order score matching'' as minimizing the objective in Eqn.~\eqref{eqn:final_objective} with $\lambda_1=\lambda_2=0$, and ``second-order score matching'' as minimizing the one with $\lambda_2=0$. Please see Appendix.~\ref{appendix:choose_lambda} for detailed settings about $\lambda_1$ and $\lambda_2$. The released code can be found at \url{https://github.com/LuChengTHU/mle_score_ode}.
\begin{remark}
\citet{song2021maximum} use a proposal distribution $t\sim p(t)$ to adjust the weighting for different time $t$ to minimize $\Jc_{\SM}(\theta)$. In our experiments, we mainly focus on the VE type, whose proposal distribution $p(t)=\Uc[0,T]$ is the same as that of our final objective in Eqn.~\eqref{eqn:final_objective}.
\end{remark}

\begin{figure}[t]
	\centering		
 	\includegraphics[width=.7\linewidth]{figures/mog_result.pdf}\\
 	\vspace{-.1in}
	\caption{$\ell_{\FISH}(t)$ and $\ell_{\SM}(t)$ of {\ode}s (VE type) on 1-D mixture of Gaussians, trained by minimizing the first, second, third-order score matching objectives.\label{fig:mog_plot}}
 	\vspace{-.1in}
\end{figure}

\begin{figure*}[t]
	\centering
	\begin{minipage}{.28\linewidth}
		\centering
			\includegraphics[width=.9\linewidth]{figures/checker_first.pdf}\\
\small{(a) First-order score matching}
	\end{minipage}
	\begin{minipage}{.28\linewidth}
	\centering
	\includegraphics[width=.9\linewidth]{figures/checker_second.pdf}\\
\small{	(b) Second-order score matching}
\end{minipage}
	\begin{minipage}{.28\linewidth}
		\centering		
 	\includegraphics[width=.9\linewidth]{figures/checker_third.pdf}\\
\small{(c) Third-order score matching}
   \end{minipage}
   \vspace{-.05in}
	\caption{Model density of {\ode}s (VE type) on 2-D checkerboard data.\label{fig:checker_density}}
	\vspace{-.15in}
\end{figure*}

\subsection{Example: 1-D Mixture of Gaussians}
\vspace{-.1cm}
\label{sec:mog_example}





We take an example to demonstrate how the high-order score matching training impacts the weighted Fisher divergence $\Jc_{\FISH}(\theta)$ and the model density of {\ode}s. Let $q_0$ be a 1-D Gaussian mixture distribution as shown in Fig.~\ref{fig:mog_intro} (a). We train a score model of VE type by minimizing the first-order score matching objective $\Jc_{\SM}(\theta)$, and use the corresponding {\ode} to evaluate the model density, as shown in Fig.~\ref{fig:mog_intro} (b). The model density achieved by only first-order score matching is quite different from the data distribution at some data points. However, by third-order score matching, the model density in Fig.~\ref{fig:mog_intro} (c) is quite similar to the data distribution, showing the effectiveness of our proposed algorithm.

We further analyze the difference of $\Jc_{\FISH}(\theta)$ between the first, second, third-order score matching training. As $q_0$ is a Gaussian mixture distribution, we can prove that each $q_t$ is also a Gaussian mixture distribution, and $\nabla_{\x}\log q_t$ can be analytically computed. Denote
\begin{align*}
    &\ell_{\FISH}(t)\!\coloneqq\! \frac{1}{2}g(t)^2\fisher{q_t}{p_t^{\ODE}},\\
    &\ell_{\SM}(t)\!\coloneqq\! \frac{1}{2}g(t)^2\E_{q_t(\x_t)}\|\s_\theta(\x_t,t)\!-\!\nabla_{\x}\!\log q_t(\x_t)\|_2^2,
\end{align*}
which are the integrands of each time $t$ for $\Jc_{\SM}(\theta)$ and $\Jc_{\FISH}(\theta)$. We use the method in Appendix.~\ref{appendix:change_of_score} to compute $\fisher{q_t}{p_t^{\ODE}}$, and evaluate $\ell_{\FISH}(t)$ and $\ell_{\SM}(t)$ from $t=\epsilon$ to $t=T$ with $100$ points of the {\ode}s trained by first, second, third-order denoising score matching objectives. As shown in Fig.~\ref{fig:mog_plot}, although $\ell_{\SM}(t)$ is small when minimizing first-order score matching objective, $\ell_{\FISH}(t)$ is rather large for most $t$, which means $\Jc_{\FISH}(\theta)$ is also large. However, the second and third score matching gradually reduce $\ell_{\FISH}(t)$, which shows that high-order score matching training can reduce $\ell_{\FISH}(t)$ and then reduce $\Jc_{\FISH}(\theta)$. Such results empirically validate that controlling the high-order score matching error can control the Fisher divergence, as proposed in Theorem~\ref{thrm:fisher_bound}.











\vspace{-.1cm}
\subsection{Density Modeling on 2-D Checkerboard Data}
\vspace{-.1cm}

We then train {\ode}s (VE type) by the first, second, third-order score matchings on the \textit{checkerboard} data whose density is multi-modal, as shown in Fig.~\ref{fig:checker_density}. We use a simple MLP neural network with Swish activations~\cite{ramachandran2017searching}, and the detailed settings are in Appendix.~\ref{appendix:checkerboard}.

For the second and third-order score matchings, we do not use any pre-trained lower-order score models. Instead, we train the score model and its first, second-order derivatives from scratch, using the objective in Eqn.~\eqref{eqn:final_objective}. The model density by the first-order score matching is rather poor, because it cannot control the value of $\nabla_{\x}\log p^{\ODE}_t$ in $\Jc_{\DIFF}(\theta)$ in Eqn.~\eqref{eqn:J_diff}. The second-order score matching can control part of $\nabla_{\x}\log p^{\ODE}_t$ and improve the model density, while the third-order score matching can reduce the Fisher divergence $\fisher{q_t}{p_t^{\ODE}}$ and achieve excellent model density. Such results show the effectiveness of our error-bounded high-order denoising score matching methods, and accord with our theoretical analysis in Theorem~\ref{thrm:kl-ode} and \ref{thrm:fisher_bound}.


\vspace{-.1cm}
\subsection{Density Modeling on Image Datasets}
\vspace{-.1cm}

We also train {\ode}s (VE type) on both the CIFAR-10 dataset~\cite{Krizhevsky09learningmultiple} and the ImageNet 32x32 dataset~\cite{deng2009imagenet}, which are two of the most popular datasets for generative modeling and likelihood evaluation. We use the estimated training objectives by trace estimators, which are detailed in Appendix.~\ref{appendix:ubiased_estimation}. We use the same neural networks and hyperparameters as the NCSN++ cont. model in~\cite{song2020score} (denoted as VE) and the NCSN++ cont. deep model in~\cite{song2020score} (denoted as VE (deep)), respectively (see detailed settings in Appendix.~\ref{appendix:cifar10} and Appendix.~\ref{appendix:imagenet32}). We evaluate the likelihood by the {\ode} $p^{\ODE}_{\epsilon}$, and sample from the {\sde} by the PC sampler~\cite{song2020score}. As shown in Table~\ref{tab:cifar10}, our proposed high-order score matching can improve the likelihood performance of {\ode}s, while retraining the high sample quality of the corresponding {\sde}s (see Appendix.~\ref{appendix:additional_samples} for samples). Moreover, the computation costs of the high-order DSM objectives are acceptable because of the trace estimators and the efficient ``Jacobian-vector-product'' computation in JAX. We list the detailed computation costs in Appendix.~\ref{appendix:cifar10}. 

We also compare the VE, VP and subVP types of ScoreODEs trained by the first-order DSM and the third-order DSM, and the detailed results are listed in Appendix.~\ref{appendix:additional_samples}.

\begin{table}
    \vspace{-.1in}
    \centering
    \caption{Negative log-likelihood (NLL) in bits/dim (bpd) and sample quality (FID scores) on CIFAR-10 and ImageNet 32x32.}
    \vskip 0.1in
    \begin{small}
    \resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{lccc}
    \toprule
    \multirow{3}{*}{Model} & \multicolumn{2}{c}{\multirow{2}{*}{CIFAR-10}} & ImageNet \Bstrut\\
    & & & 32x32\\
    \cline{2-4}
    & NLL $\downarrow$ & FID $\downarrow$ & NLL $\downarrow$ \Tstrut\\
    \midrule
        VE~\cite{song2020score} & 3.66 & 2.42 & 4.21\\
        VE (second)~(\bf{ours}) & 3.44 & \textbf{2.37} & 4.06\\
        VE (third)~(\bf{ours}) & \bf{3.38} & 2.95 & \textbf{4.04}\Bstrut\\
    \hline
        VE (deep)~\cite{song2020score} & 3.45 & \textbf{2.19} & 4.21\Tstrut \\
        VE (deep, second)~(\bf{ours}) & 3.35 & 2.43 & 4.05\\
        VE (deep, third)~(\bf{ours}) & \bf{3.27} & 2.61 & \textbf{4.03}\\
    \bottomrule
    \end{tabular}%
    }
    \end{small}
    \label{tab:cifar10}
    \vspace{-0.15in}
\end{table}



==> fgkgtjmwskwbymryhxmxswbkzvkyvmcj/common.tex <==
\usepackage{color}
\usepackage{bm}
\usepackage{hyperref}
\usepackage{amsmath,amsfonts}
\usepackage{blindtext}
\usepackage{listings}
\usepackage{mathtools}

\newif\ifdebug
\debugtrue

\newcommand{\lc}[1]{{\color{red}{[lc: #1]}}}
\newcommand{\sde}{ScoreSDE}
\newcommand{\ode}{ScoreODE}

\newcommand{\FISH}{\text{Fisher}}
\newcommand{\DSM}{\text{DSM}}
\newcommand{\SM}{\text{SM}}
\newcommand{\DIFF}{\text{Diff}}
\newcommand{\SDE}{\text{SDE}}
\newcommand{\ODE}{\text{ODE}}
\newcommand{\Lip}{\mathrm{Lip}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\logdet}[1]{\log\left|#1\right|}


\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
	#1\;\delimsize\|\;#2%
}
\newcommand{\infdiv}{D\infdivx}
\newcommand{\kl}{D_{\mathrm{KL}}\infdivx}
\newcommand{\fisher}{D_{\mathrm{F}}\infdivx}


\newcommand{\vect}[1]{\bm{#1}}

\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}

\newcommand{\x}{\xv}
\newcommand{\y}{\yv}
\newcommand{\z}{\zv}
\newcommand{\s}{\sv}
\newcommand{\rv}{\vect{r}}
\newcommand{\dm}{\mathrm{d}}

\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\Bern}{\mbox{Bern}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\Mult}{\mbox{Mult}}
\newcommand{\Dice}{\mbox{Dice}}
\newcommand{\Cat}{\mbox{Cat}}
\newcommand{\dx}{\mathrm{d}x}
\newcommand{\dxv}{\mathrm{d}\xv}
\newcommand{\dy}{\mathrm{d}y}
\newcommand{\dyv}{\mathrm{d}\yv}
\newcommand{\dzv}{\mathrm{d}\zv}
\newcommand{\dwv}{\mathrm{d}\wv}
\newcommand{\dt}{\mathrm{d}t}
\newcommand{\dlog}{\mathrm{d}\log}

\newcommand{\alphav}{\vect\alpha}
\newcommand{\betav}{\vect\beta}
\newcommand{\gammav}{\vect\gamma}
\newcommand{\deltav}{\vect\delta}
\newcommand{\epsilonv}{\vect\epsilon}
\newcommand{\zetav}{\vect\zeta}
\newcommand{\etav}{\vect\eta}
\newcommand{\thetav}{\vect\theta}
\newcommand{\iotav}{\vect\iota}
\newcommand{\kappav}{\vect\kappa}
\newcommand{\lambdav}{\vect\lambda}
\newcommand{\muv}{\vect\mu}
\newcommand{\nuv}{\vect\nu}
\newcommand{\xiv}{\vect\xi}
\newcommand{\omicronv}{\vect\omicron}
\newcommand{\piv}{\vect\pi}
\newcommand{\rhov}{\vect\rho}
\newcommand{\sigmav}{\vect\sigma}
\newcommand{\tauv}{\vect\tau}
\newcommand{\upsilonv}{\vect\upsilon}
\newcommand{\phiv}{\vect\phi}
\newcommand{\chiv}{\vect\chi}
\newcommand{\psiv}{\vect\psi}
\newcommand{\omegav}{\vect\omega}
\newcommand{\varphiv}{\vect\varphi}

\newcommand{\Alphav}{\vect\Alpha}
\newcommand{\Betav}{\vect\Beta}
\newcommand{\Gammav}{\vect\Gamma}
\newcommand{\Deltav}{\vect\Delta}
\newcommand{\Epsilonv}{\vect\Epsilon}
\newcommand{\Zetav}{\vect\Zeta}
\newcommand{\Etav}{\vect\Eta}
\newcommand{\Thetav}{\vect\Theta}
\newcommand{\Iotav}{\vect\Iota}
\newcommand{\Kappav}{\vect\Kappa}
\newcommand{\Lambdav}{\vect\Lambda}
\newcommand{\Muv}{\vect\Mu}
\newcommand{\Nuv}{\vect\Nu}
\newcommand{\Xiv}{\vect\Xi}
\newcommand{\Omicronv}{\vect\Omicron}
\newcommand{\Piv}{\vect\Pi}
\newcommand{\Rhov}{\vect\Rho}
\newcommand{\Sigmav}{\vect\Sigma}
\newcommand{\Tauv}{\vect\Tau}
\newcommand{\Upsilonv}{\vect\Upsilon}
\newcommand{\Phiv}{\vect\Phi}
\newcommand{\Chiv}{\vect\Chi}
\newcommand{\Psiv}{\vect\Psi}
\newcommand{\Omegav}{\vect\Omega}
\newcommand{\Varphiv}{\vect\Varphi}

\newcommand{\av}{\vect a}
\newcommand{\bv}{\vect b}
\newcommand{\cv}{\vect c}
\newcommand{\fv}{\vect f}
\newcommand{\gv}{\vect g}
\newcommand{\hv}{\vect h}
\newcommand{\iv}{\vect i}
\newcommand{\jv}{\vect j}
\newcommand{\kv}{\vect k}
\newcommand{\lv}{\vect l}
\newcommand{\ellv}{\vect \ell}
\newcommand{\mv}{\vect m}
\newcommand{\nv}{\vect n}
\newcommand{\ov}{\vect o}
\newcommand{\qv}{\vect q}
\newcommand{\sv}{\vect s}
\newcommand{\tv}{\vect t}
\newcommand{\uv}{\vect u}
\newcommand{\vv}{\vect v}
\newcommand{\wv}{\vect w}
\newcommand{\xv}{\vect x}
\newcommand{\yv}{\vect y}
\newcommand{\zv}{\vect z}

\newcommand{\Av}{\vect A}
\newcommand{\Bv}{\vect B}
\newcommand{\Cv}{\vect C}
\newcommand{\Dv}{\vect D}
\newcommand{\Ev}{\vect E}
\newcommand{\Fv}{\vect F}
\newcommand{\Gv}{\vect G}
\newcommand{\Hv}{\vect H}
\newcommand{\Iv}{\vect I}
\newcommand{\Jv}{\vect J}
\newcommand{\Kv}{\vect K}
\newcommand{\Lv}{\vect L}
\newcommand{\Mv}{\vect M}
\newcommand{\Nv}{\vect N}
\newcommand{\Ov}{\vect O}
\newcommand{\Pv}{\vect P}
\newcommand{\Qv}{\vect Q}
\newcommand{\Rv}{\vect R}
\newcommand{\Sv}{\vect S}
\newcommand{\Tv}{\vect T}
\newcommand{\Uv}{\vect U}
\newcommand{\Vv}{\vect V}
\newcommand{\Wv}{\vect W}
\newcommand{\Xv}{\vect X}
\newcommand{\Yv}{\vect Y}
\newcommand{\Zv}{\vect Z}

\newcommand{\Ac}{\mathcal A}
\newcommand{\Bc}{\mathcal B}
\newcommand{\Cc}{\mathcal C}
\newcommand{\Dc}{\mathcal D}
\newcommand{\Ec}{\mathcal E}
\newcommand{\Fc}{\mathcal F}
\newcommand{\Gc}{\mathcal G}
\newcommand{\Hc}{\mathcal H}
\newcommand{\Ic}{\mathcal I}
\newcommand{\Jc}{\mathcal J}
\newcommand{\Kc}{\mathcal K}
\newcommand{\Lc}{\mathcal L}
\newcommand{\Mc}{\mathcal M}
\newcommand{\Nc}{\mathcal N}
\newcommand{\Oc}{\mathcal O}
\newcommand{\Pc}{\mathcal P}
\newcommand{\Qc}{\mathcal Q}
\newcommand{\Rc}{\mathcal R}
\newcommand{\Sc}{\mathcal S}
\newcommand{\Tc}{\mathcal T}
\newcommand{\Uc}{\mathcal U}
\newcommand{\Vc}{\mathcal V}
\newcommand{\Wc}{\mathcal W}
\newcommand{\Xc}{\mathcal X}
\newcommand{\Yc}{\mathcal Y}
\newcommand{\Zc}{\mathcal Z}


\newcommand{\Ab}{\mathbb A}
\newcommand{\Bb}{\mathbb B}
\newcommand{\Cb}{\mathbb C}
\newcommand{\Db}{\mathbb D}
\newcommand{\Eb}{\mathbb E}
\newcommand{\Fb}{\mathbb F}
\newcommand{\Gb}{\mathbb G}
\newcommand{\Hb}{\mathbb H}
\newcommand{\Ib}{\mathbb I}
\newcommand{\Jb}{\mathbb J}
\newcommand{\Kb}{\mathbb K}
\newcommand{\Lb}{\mathbb L}
\newcommand{\Mb}{\mathbb M}
\newcommand{\Nb}{\mathbb N}
\newcommand{\Ob}{\mathbb O}
\newcommand{\Pb}{\mathbb P}
\newcommand{\Qb}{\mathbb Q}
\newcommand{\Rb}{\mathbb R}
\newcommand{\Sb}{\mathbb S}
\newcommand{\Tb}{\mathbb T}
\newcommand{\Ub}{\mathbb U}
\newcommand{\Vb}{\mathbb V}
\newcommand{\Wb}{\mathbb W}
\newcommand{\Xb}{\mathbb X}
\newcommand{\Yb}{\mathbb Y}
\newcommand{\Zb}{\mathbb Z}

\newcommand{\inorm}[1]{\norm{#1}_\infty}
\newcommand{\iprod}[1]{\langle#1\rangle}

\newcommand{\splitop}{\mbox{split}}
\newcommand{\concat}{\mbox{concat}}

\newcommand{\cvloss}{f_{CV, v}}
\newcommand{\loss}{f_v}
\newcommand{\ZL}{Z^{(l)}}
\newcommand{\ZLp}{Z^{(l+1)}}
\newcommand{\HL}{H^{(l)}}
\newcommand{\HLp}{H^{(l+1)}}
\newcommand{\scv}{_{CV}}
\newcommand{\ZLcv}{\ZL\scv}
\newcommand{\ZLpcv}{\ZLp\scv}
\newcommand{\HLcv}{\HL\scv}
\newcommand{\HLpcv}{\HLp\scv}
\newcommand{\WL}{W^{(l)}}
\newcommand{\WLT}{W^{(l)\top}}
\newcommand{\PhL}{\hat P^{(l)}}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\Cov}{\mbox{Cov}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\Diag}{\mbox{Diag}}

\newcommand{\bl}{{(l)}}
\newcommand{\bll}{{(l+1)}}
\newcommand{\bL}{{(L)}}
\newcommand{\NS}{\mbox{NS}}
\newcommand{\CV}{\mbox{CV}}
\newcommand{\CVD}{\mbox{CVD}}
\newcommand{\Ideal}{\mbox{Ideal}}
\newcommand{\nbr}{\Nc(u)}
\newcommand{\snbr}{\hat \Nc^\bl(u)}







\newcommand{\hst}{\hat \sv_t}
\newcommand{\hstt}{\hat \sv_{t+1}}
\newcommand{\Dfhst}{\Delta \fv_i(\hst)}
\newcommand{\bfhst}{\bar \fv(\hst)}
\newcommand{\bfhstt}{\bar \fv(\hstt)}
\newcommand{\bhstt}{\bar \sv_{t+1}}
\newcommand{\hess}[1]{\nabla^2_{#1} \fv(#1)}
\newcommand{\lmax}{\lambda_{\mbox{max}}}
\newcommand{\lmin}{\lambda_{\mbox{min}}}
\newcommand{\hsz}{\hat \sv_0}
\newcommand{\Uniform}{\mbox{Uniform}}


\DeclareMathOperator{\sign}{sign}





	

